Defending against Machine Learning based Inference Attacks via Adversarial Examples: Opportunities and Challenges

As machine learning (ML) becomes more and more powerful and easily accessible, attackers increasingly leverage ML to perform automated large-scale inference attacks in various domains. In such an ML-equipped inference attack, an attacker has access to some data (called public data) of an individual, a software, or a system; and the attacker uses an ML classifier to automatically infer their private data. Inference attacks pose severe privacy and security threats to individuals and systems. Inference attacks are successful because private data are statistically correlated with public data, and ML classifiers can capture such statistical correlations. In this chapter, we discuss the opportunities and challenges of defending against ML-equipped inference attacks via adversarial examples. Our key observation is that attackers rely on ML classifiers in inference attacks. The adversarial machine learning community has demonstrated that ML classifiers have various vulnerabilities. Therefore, we can turn the vulnerabilities of ML into defenses against inference attacks. For example, ML classifiers are vulnerable to adversarial examples, which add carefully crafted noise to normal examples such that an ML classifier makes predictions for the examples as we desire. To defend against inference attacks, we can add carefully crafted noise into the public data to turn them into adversarial examples, such that attackers' classifiers make incorrect predictions for the private data. However, existing methods to construct adversarial examples are insufficient because they did not consider the unique challenges and requirements for the crafted noise at defending against inference attacks. In this chapter, we take defending against inference attacks in online social networks as an example to illustrate the opportunities and challenges.

==> abstract.tex <==
\begin{abstract}
Users in various web and mobile applications are vulnerable to \emph{attribute inference attacks}, in which an attacker leverages a machine learning classifier to infer a target user's private attributes (e.g., location, sexual orientation, political view) from its public data (e.g., rating scores, page likes). 
Existing defenses leverage game theory or heuristics based on correlations between the public data and attributes. These defenses are not practical. 
Specifically, game-theoretic defenses require solving intractable optimization problems,  %because of the high dimensionality of the public data in practice, 
while correlation-based defenses incur large utility loss of users' public data. %achieve sub-optimal privacy-utility tradeoffs.   


In this paper, we present \emph{AttriGuard}, a practical defense against attribute inference attacks. AttriGuard is computationally tractable and has small utility loss.  Our AttriGuard works in two phases. Suppose we aim to protect a user's private attribute. In Phase I, for each value of the attribute, we find a minimum noise such that if we add the noise to the user's public data, then the attacker's classifier is very likely to infer the attribute value for the user. We find the minimum noise via adapting existing \emph{evasion attacks} in adversarial machine learning. In Phase II, we sample one attribute value according to a certain probability distribution and add the corresponding noise found in Phase I to the user's public data. We formulate finding the probability distribution as solving a constrained convex optimization problem. We extensively evaluate AttriGuard and compare it with existing methods using a real-world dataset. Our results show that AttriGuard substantially outperforms existing methods.  Our work is the first one that shows evasion attacks can be used as defensive techniques for privacy protection. 

%we can mitigate attribute inference attacks with a small utility loss; adversarial machine learning can play an important role at protecting users from attribute inference attacks; and our defense substantially outperforms existing methods. 


%First, we formally define the problem of defending against MaLIA. The defender adds noise to a user's public data according to a mechanism, which is obtained via solving the optimization problems that we formulate to achieve optimal privacy-utility tradeoffs. Second, we propose a two-phase framework called \emph{MaLIAGuard} to solve the formulated inference-attack defense problems. In particular, in Phase I of our framework, we compute the noises needed to evade the attacker's classifier, which can be viewed as \emph{evasion attacks} in adversarial machine learning. 
%Third, we extensively evaluate MaLIAGuard and compare it with existing methods using a real-world dataset. Our results demonstrate that we can mitigate MaLIA with a small utility loss; adversarial machine learning can play an important role at protecting users from MaLIA; and our framework substantially outperforms existing methods. 


%In particular, in Phase I, we compute noises that can be added to a user's public data 


%In this paper, we explore how to defend against statistical inference attack using released data to predict undisclosed private information about individuals. 
%We propose an general privacy preserving framework(APSI) to defend against statistical inference attack using information-theoretic as well as adversarial machine learning.
%In our system, each user perturbs her data locally before sending the noisy data to the data collector. 
%Our system don't need assumption of trusted third-party server which is impractical in real world application.
%
%We use google plus app rating datasets to evaluate our system, we show that by add relative small noise, we can protect user's privacy with lower information leakage.
\end{abstract}

==> exp.tex <==

\section{Evaluation}
\label{exp}



\subsection{Experimental Setup}

\subsubsection{Dataset} 
We obtained a review dataset from Gong and Liu~\cite{GongAttriInferSEC16}. The public data of a user are the Google Play apps the user rated. We selected 10,000 popular apps and kept the users who reviewed at least 10 apps. 
In total, we have 16,238 users, and each user rated 23.2 apps on average. We represent a user's public data as a 10,000-dimension vector $\mathbf{x}$, where each entry corresponds to an app. If the user rated an app, the corresponding entry is the rating score (i.e., 1, 2, 3, 4, or 5),  %if the user liked an app, the corresponding entry has a value of 5; and 
otherwise the corresponding entry has a value of 0. The attribute is the city a user lives/lived in, which were collected from users' Google+ profiles and obtained from Gong et al.~\cite{Gong12-imc}.  In total, we consider 25 popular cities. Figure~\ref{citypopu} shows the fraction of users that live/lived in a particular city. Note that we normalize each entry of a user's public data vector (i.e., review data vector) to be in [0,1], i.e., each entry is 0, 0.2, 0.4, 0.6, 0.8, or 1.0.
 
\myparatight{Training and testing} We sample 90\% of the users in the dataset uniformly at random and assume that they publicly disclose their cities lived, e.g., on Google+. The app review data and lived cities of these users are called \emph{training dataset}.  The remaining users do not disclose their cities lived, and we call them \emph{testing dataset}. 



% \begin{table}[!t]\renewcommand{\arraystretch}{1.2}
%\centering
% \caption{Dataset statistics.}
% %\centering
% %\addtolength{\tabcolsep}{-4pt}
% \begin{tabular}{|c|c|c|c|} \hline 
% { \textbf{\#Users}} & { \textbf{\#Ave. App}} & { \textbf{\#City}} \\ \hline 
% { 16,238} & { 23.24} & { 25}  \\ \hline
% \end{tabular} \\
% %\vspace{-.1in}
% \label{dataset} 
% \end{table}

\begin{figure}[!t]
%\vspace{-2mm}
\centering
%\includegraphics[width=0.38 \textwidth]{figs/Figure1/Fraction_of_user.pdf}
\includegraphics[scale=.38]{figs/Figure1/Fraction_of_user.pdf}
%\subfloat[Recall]{\includegraphics[width=0.25 \textwidth]{lr_minkl.pdf} \label{recall}}
%\subfloat[Recall]{\includegraphics[width=0.25 \textwidth]{number_of_app_added_prior.pdf} \label{f-score}}
\caption{Fraction of users who live/lived in a city.}
%We observe that backtracking substantially improves VIAL's performance. }
%Second, we find that inference performances are stable across  different backtracking strengths once they are larger than 0.}
\vspace{-4mm}
\label{citypopu}
\end{figure}



\subsubsection{Attribute Inference Attacks} 
An attribute inference attack aims to infer the cities lived for the testing users. Specifically, an attacker learns a multi-class classifier, which takes a review data vector as an input and infers the city lived, using the training dataset. We evaluate an attack using the \emph{inference accuracy} of the classifier used by the attack. Formally, 
 the {inference accuracy} of a classifier is the fraction of testing users that the inferred city lived is correct.
%Moreover, we aim to leverage our AttriGuard to defend against the attribute inference attacks for these test users. 
Since the defender does not know the attacker's classifier, we evaluate the effectiveness of AttriGuard against various attribute inference attacks as follows (we use a suffix ``-A" to indicate the classifiers are used by the attacker): 

%\begin{packeditemize}
\myparatight{Baseline attack (BA-A)} In this baseline attack, the attacker computes the most popular city among the users in the training dataset. The attacker predicts the most popular city for every user in the testing dataset. The inference accuracy of this baseline attack will not be changed by defenses that add noise to the testing users.  


\myparatight{Logistic regression (LR-A)} In this attack, the attacker uses a multi-class logistic regression classifier to perform attribute inference attacks. The LR classifier was also used by previous attribute inference attacks~\cite{kosinski2013private,weinsberg2012blurme,GongAttriInferSEC16,AttriInfer}.

%\item {\bf Support vector machine (SVM).} In this attack, the attacker uses a SVM classifier to perform attacks.  

\myparatight{Random forest (RF-A)} In this attack, the attacker uses a random forest classifier to perform attacks.  

\myparatight{Neural network (NN-A)}  We consider the attacker uses a three-layer (i.e., input layer, hidden layer, and output layer) fully connected neural network to perform attacks. %We denote the classifier as NN-A to distinguish with the neural network classifier NN-D used by the defender. 
The hidden layer has 30,000 neurons. The output layer is a softmax layer.
We adopt the \emph{rectified linear units} as the activation function for neurons as it was demonstrated to outperform other activation functions~\cite{ReLU}. 
Note that the three-layer NN-A classifier might not be the best neural network classifier for inferring the city lived. However, exploring the best NN-A is not the focus of our work.
%We note that, we also explored more complex neural networks such as deep convolutional neural networks. However, the inference accuracy decreases or is close to that achieved by the three-layer neural network. One possible reason is that deep neural networks require a large amount of training data, which is not the case in our setting. 

%\myparatight{VIAL-A~\cite{GongAttriInferSEC16}}  Gong and Liu~\cite{GongAttriInferSEC16} proposed a graph-based attribute inference attack called VIAL, which uses social friends and/or behavior data. We consider the variant of VIAL that only leverages behavior data, i.e., app reviews in our setting. Essentially, VIAL-A constructs a tripartite graph between users, apps, and cities; and then VIAL-A uses random walks to perform attribute inference.   

\myparatight{Robust classifiers: adversarial training (AT-A), defensive distillation (DD-A), and region-based classification (RC-A)} Since our defense AttriGuard leverages adversarial examples to find the noise, an attacker could leverage classifiers that are more robust to adversarial examples, based on the knowledge of our defense. We consider robust classifiers based on adversarial training~\cite{Goodfellow:ICLR:14b}, defensive distillation~\cite{Papernot16Distillation}, and region-based classification~\cite{region}. In adversarial training, an attacker generates noise for each user in the training dataset using AttriGuard and learns the neural network classifier NN-A using the noisy training dataset. In defensive distillation, an attacker refines its neural network classifier NN-A using soft labels. In region-based classification, for each testing user with a certain review data vector, an attacker randomly samples $n$ data points from a hypercube centered at the review data vector; applies the NN-A classifier to predict the attribute for each sampled data point; and the attacker takes a majority vote among the sampled data points to infer the user's attribute. We set $n=100$.  
%Figure~\ref{adaptedMA} also includes the inference accuracy for such adapted MaLIAs when MaLIAGuard generates noise based on a standard MaLIA. We observe that when privacy-risk budget is large, the adapted MaLIAs just have slightly higher inference accuracy than the standard MaLIA. In other words, to make the attacker achieve the same inference accuracy, MaLIAGuard needs to add slightly more noises to the public data. We believe that robust classifiers will influence the privacy-utility tradeoff, i.e., MaLIAGuard needs to add more noises to achieve the same privacy guarantee when the attacker uses robust classifiers. However, such influence may be small. 

\myparatight{Detecting noise via low-rank approximation (LRA-A)} An attacker could detect noise, remove the noise, and then perform attribute inference attacks. Whether the noise added by AttriGuard can be detected by an attacker and how to detect it effectively are not the focuses of this work, though we believe they are interesting future works. In this work, we try one way of detecting noise. 
An attacker essentially obtains a matrix of (noisy) public data for users, where each row corresponds to a user. Each entry of the matrix is a rating score or 0 if the corresponding user did not rate the item. It was well known that, in recommender systems, a normal rating-score matrix can be explained by a small number of latent factors. Therefore, 
an attacker could perform a \emph{low-rank approximation (LRA)} of the matrix. After low-rank approximation, each row could be viewed as the de-noised rating scores of a user. Then, the attacker uses these de-noised rating scores to learn a classifier NN-A and uses it to perform attribute inference.      
We implemented LRA using non-negative matrix factorization with a rank 500.
%Figure~\ref{adaptedMA} (the curve ``LRA-based MaLIA'') shows the inference accuracy of the LRA-based adapted MaLIA when MaLIAGuard adds noise based on a standard MaLIA (the classifier is NN). We observe that this   LRA-based adapted MaLIA achieves even worse inference accuracy. While our results demonstrate the ineffectiveness of LRA-based noise detection, it does not necessarily mean that an attacker cannot detect noises. We believe it is an interesting future work to study whether and how an attacker can detect the noises and adapt MaLIAs both theoretically and empirically. We note that detecting noises is different from \emph{detecting adversarial examples}~\cite{detection1,detection2,xu2017feature,liang2017detecting} in adversarial machine learning, because detecting adversarial examples is to detect whether a given example has attacker-added noise or not.   


%\end{packeditemize}

\begin{table}[!t]\renewcommand{\arraystretch}{1}
\centering
\caption{Inference accuracy of different attribute inference attacks when no defense is used.}
%\centering
%\addtolength{\tabcolsep}{-4pt}
%\vspace{-1mm}
\begin{tabular}{|c|c|} \hline 
%\multirow{2}{*}{Classifier} &
Attack & Inference Accuracy \\ \hline
BA-A & 0.10 \\ \hline
LR-A & 0.43 \\ \hline
RF-A & 0.44 \\ \hline
NN-A & 0.39 \\ \hline
%VIAL-A & 0.42 \\ \hline
AT-A & 0.39 \\ \hline
DD-A & 0.40 \\ \hline
RC-A & 0.38 \\ \hline
LRA-A & 0.27\\ \hline
\end{tabular} 
%\vspace{-2mm}
\label{inferAcc} 
\end{table}

%\begin{figure}[!t]
%%\vspace{-2mm}
%\centering
%%\subfloat[]{\includegraphics[width=0.45 \textwidth]{figs/Figure4/Figure4a.pdf}\label{up1}}
%%\subfloat[]
%{\includegraphics[scale=0.4]{figs/Figure13/RC.pdf}}
%\caption{Inference accuracy vs. radius of the hypercube for RC-A.}
%%We observe that backtracking substantially improves VIAL's performance. }
%%Second, we find that inference performances are stable across  different backtracking strengths once they are larger than 0.}
%\vspace{-2mm}
%\label{rc}
%\end{figure}


The attacks BA-A, LR-A, RF-A, and NN-A are unaware of the defense, while AT-A, DD-A, RC-A, and LRA-A are attacks that adapt to defense. 
Table~\ref{inferAcc} shows the inference accuracy of each attack for the testing users when no defense is used. 
We note that RC-A's inference accuracy depends on the radius of the hypercube. 
%Figure~\ref{rc} shows the inference accuracy as a function of the radius for RC-A. 
%After 0.05, the inference accuracy drops sharply. Therefore, 
We set the radius to be 0.05 in our experiments as the inference accuracy drops sharply after that~\cite{AttriGuard}. 
Unless otherwise mentioned, we assume the attacker uses NN-A because it is harder for the defender to guess the neural network setting. 
 Gong and Liu~\cite{GongAttriInferSEC16} proposed an attribute inference attack. However, their attack requires both social friends and behavior data. Since our work focuses on attribute inference attacks that only use behavior data (i.e., app review data in our experiments), we do not compare with their attack.



\subsubsection{Parameter Setting in AttriGuard} 
The defender aims  to protect the cities lived for the testing users. 

\myparatight{Target probability distribution $\mathbf{p}$} We consider two target probability distributions. 
\begin{itemize}
\item {\bf Uniform probability distribution $\mathbf{p}_u$.} Without any information about the cities lived, the target probability distribution (denoted as $\mathbf{p}_u$) could be the uniform probability distribution over the 25 cities, with which the defender aims to minimize the difference between an attacker's inference and random guessing subject to a utility-loss budget. 
\item {\bf Training-dataset-based $\mathbf{p}_t$.}  The defender can also estimate the target probability distribution (denoted as $\mathbf{p}_t$) from the training dataset. Specifically, the target probability for city $i$ is the fraction of training users who have city $i$. With such target probability distribution, the defender aims to minimize the difference between an attacker's inference and the baseline attack BA-A. 
\end{itemize}

Unless otherwise mentioned, we assume the defender uses the second target probability distribution $\mathbf{p}_t$ since it considers certain knowledge about the attributes. 


\myparatight{Defender's classifier $C$ (LR-D and NN-D)}  We consider two choices for the defender's classifier, i.e., multi-class logistic regression (LR-D) and neural network (NN-D). 
To distinguish between the classifiers used by the attacker and those used by the defender, we use a suffix ``-A" for each attacker's classifier while we use a suffix ``-D" for a defender's classifier.  
We note that the defender could choose any differentiable classifier. We require differentiable classifiers because our algorithm PANDA in Phase I is applicable to differentiable classifiers. For the NN-D classifier, we also consider a three-layer fully connected neural network. However, unlike NN-A that is used by the attacker, we assume the hidden layer of the NN-D classifier has 50,000 neurons. Unless otherwise mentioned, we assume the defender uses the LR-D classifier and learns it using the training dataset. We adopt LR-D as the default classifier because it is much more efficient to generate noise in Phase I. We will study the effectiveness of our defense when the attacker and the defender use different dataset to learn their classifiers.  

\myparatight{Other parameters} We set $\tau$ in our algorithm PANDA to be 1.0 when finding the minimum noise. %How to normalize them to be  0.2,0.4, ...
Unless otherwise mentioned, we set the noise-type-policy to be Modify\_Add. 

 
  \begin{figure}[!t]
%\vspace{-2mm}
\centering
\subfloat[LR-D]{\includegraphics[scale=0.33]{figs/Figure2/city_appadded_lr.pdf}}
\subfloat[NN-D]{\includegraphics[scale=0.33]{figs/Figure2/city_appadded_nn.pdf}}
%\subfloat[Recall]{\includegraphics[width=0.25 \textwidth]{lr_minkl.pdf} \label{recall}}
%\subfloat[Recall]{\includegraphics[width=0.25 \textwidth]{city_appadded_lr_0.pdf} \label{f-score}}
\caption{Average noise for each city. The defender's classifier is (a) LR-D and (b) NN-D, respectively.}
%We observe that backtracking substantially improves VIAL's performance. }
%Second, we find that inference performances are stable across  different backtracking strengths once they are larger than 0.}
%\vspace{-4mm}
\label{noise}
\end{figure}


 \begin{table}[!t]\renewcommand{\arraystretch}{1}
\centering
\caption{Average success rates and running times.}
%\centering
%\addtolength{\tabcolsep}{-4pt}
%\vspace{-1mm}
\begin{tabular}{|c|c|c|c|c|} \hline 
%\multirow{2}{*}{Classifier} &
 \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Success Rate} & \multicolumn{2}{c|}{Running Time (s)} \\ \cline{2-5} 
&LR-D & NN-D & LR-D & NN-D \\ \hline
{ {FGSM}} & {  100\%} & 100\% &  {7.6} & 84 \\ \hline
{ {JSMA}} & {  100\%}& {  100\%} & {9.0}& {295}  \\ \hline
{ {CW}} & { 75\%} & { 71\%} & {7,406} & {1,067,610} \\ \hline
{ {PANDA}} & { 100\%} & { 100\%} & {8.7} & {272}  \\ \hline
% & { {JSMA}} & { 100\%} & {295}  \\ \cline{2-4}
% & { {SA}} & { 71\%} & {1,067,610}  \\ \cline{2-4}
% & { {PANDA}} & { 100\%} & {272}  \\ \hline
% \multirow{4}{*}{LR}& { {FGS}} & {  100\%} & {7.6}  \\ \cline{2-4}
%& { {JSMA}} & {  100\%} & {9.0}  \\ \cline{2-4}
%& { {SA}} & { 75\%} & {7,406}  \\ \cline{2-4}
% & { {PANDA}} & { 100\%} & {8.7}  \\ \hline\hline
% \multirow{4}{*}{NN} & { {FGS}} & { 100\%} & {84}  \\ \cline{2-4}
% & { {JSMA}} & { 100\%} & {295}  \\ \cline{2-4}
% & { {SA}} & { 71\%} & {1,067,610}  \\ \cline{2-4}
% & { {PANDA}} & { 100\%} & {272}  \\ \hline
\end{tabular} 
%\vspace{-2mm}
\label{comp_method} 
\end{table}

 
 \subsection{Results}



\myparatight{Comparing PANDA with existing adversarial example methods} %For each test user, 
%Phase I of AttriGuard uses PANDA to find minimum noise $\mathbf{r}_i$ for each city such that the defender-selected classifier infers the $i$th city for the test user when taking the noisy public data as an input. 
We compare PANDA with the following adversarial example methods at finding the noise $\mathbf{r}_i$ in Phase I: \emph{Fast Gradient Sign Method} (FGSM)~\cite{Goodfellow:ICLR:14b}, \emph{Jacobian-based Saliency Map Attack} (JSMA)~\cite{Papernot:arxiv:16Limitation}, and \emph{Carlini and Wagner Attack} (CW)~\cite{CarliniSP17}. In each iteration of JSMA, we only pick one entry of the public data vector to modify, because searching for the optimal two entries is inefficient. We leveraged the open-source implementation of CW published by its authors. 
%Note that JSMA has two versions: one version uses the softmax outputs (JSMA-F), and the other version uses the inputs to the softmax layer (JSMA-Z). We found that JSMA-F works better than JSMA-Z in our problem, so we will show results on JSMA-F. 
%CW shrinks the set of entries that are modified by greedily searching for optimal parameter configuration.  
The CW attack has three variants that are optimized to find small noise measured by $L_0$, $L_2$, and $L_\infty$ norms, respectively. We use the one that optimizes $L_0$ norm.
%Carlini and Wagner~\cite{CarliniSP17} proposed three versions of attacks that are optimized for $L_0$, $L_2$, and $L_\infty$, respectively. CW is the one that optimizes $L_0$ norm. 
We focus on the noise-type-policy Modify\_Add, because FGSM, JSMA, and CW are not applicable to other policies. 
Note that after a method produces a noise $\mathbf{r}_i$, we will round each entry to be 0, 0.2, 0.4, 0.6, 0.8, or 1.0 since our noisy public data are discrete rating scores, and the rounded $\mathbf{r}_i$ is treated as the final noise.  


Figure~\ref{noise} shows their noise (measured by $L_0$ norm) averaged over test users for each city. Moreover, Table~\ref{comp_method} shows the \emph{success rate} and \emph{running time} averaged over test users for each compared method. For each method, a test user's success rate is the fraction of cities for which the method can successfully find a $\mathbf{r}_i$ to make the classifier infer the $i$th city for the test user, and a test user's running time is the time required for the method to find $\mathbf{r}_i$ for all cities. We set the step size parameter $\epsilon$ in FGSM to be 1 as we aim to achieve a high success rate. Note that the value of $\epsilon$ does not impact the $L_0$ norm of the noise generated by FGSM. 


\begin{figure}[!t]
%\vspace{-2mm}
\centering
%\subfloat[]{\includegraphics[width=0.45 \textwidth]{figs/Figure4/Figure4a.pdf}\label{up1}}
%\subfloat[]
{\includegraphics[scale=0.4]{figs/Figure3/Figure3-2.pdf}}
\caption{Attacker's inference accuracy vs. utility-loss budget.}
%We observe that backtracking substantially improves VIAL's performance. }
%Second, we find that inference performances are stable across  different backtracking strengths once they are larger than 0.}
%\vspace{-4mm}
\label{up}
\end{figure}

First, FGSM adds orders of magnitude larger noise than other methods. This is because FGSM aims to minimize noise with respect to $L_\infty$ norm instead of $L_0$ norm.
Second, PANDA adds smaller noise and is slightly faster than JSMA for both LR-D and NN-D classifiers. This is because PANDA allows more flexible noise, i.e., some entries can be increased while other entries can be decreased in PANDA, while all modified entries can either be increased or decreased in JSMA. PANDA is faster than JSMA because it adds smaller noise and thus it runs for less iterations. Third, PANDA adds no larger noise than CW for the LR-D classifier; and PANDA adds smaller noise for some cities, but larger noise for other cities for the NN-D classifier. However, CW only has success rates less than 80\%, because of rounding the noise to be consistent with rating scores.  
 Moreover, PANDA is around 800 times and 4,000 times faster than CW for the LR-D and NN-D classifiers, respectively.  %In practice, when a user rates a new app, our framework needs to add new noise to re-achieve a privacy-utility tradeoff (see our experiments on \emph{dynamic public data} at the end of this section). Therefore, the method of finding the noises should be efficient in order to provide real-time defense service. 
 Considering the tradeoffs between the added noise, success rate, and running time, we recommend to use PANDA for finding noise in Phase I of AttriGuard. 

We note that JSMA and CW have similar noise for the LR-D classifier, and CW even has larger noise than JSMA for certain cities for the NN-D classifier.  Carlini and Wagner~\cite{CarliniSP17} found that CW outperforms JSMA. We suspect the reason is that our results are on review data, while their results are about image data.  




\myparatight{AttriGuard is effective} Figure~\ref{up} shows the inference accuracy of various attribute inference attacks as the utility-loss budget increases, where the defender's classifier is LR-D. AttriGuard is effective at defending against attribute inference attacks. For instance, when modifying 3-4 rating scores on average, several attacks become less effective than the baseline attack. The inference accuracy of LR-A decreases the fastest as the utility-loss budget increases. This is because the defender uses LR-D, and the noise optimized based on LR-D is more likely to transfer to LR-A. The adversarial training attack AT-A has almost the same inference accuracy as NN-A. The reason is that adversarial training is not robust to iterative adversarial example methods~\cite{AT17} and PANDA is an iterative adversarial example method. Defensive distillation attack DD-A has slightly higher inference accuracies than NN-A, because defensive distillation is more robust to the saliency map based adversarial examples~\cite{Papernot16Distillation}. LRA-A is more robust to the noise added by AttriGuard, i.e., the inference accuracy of LRA-A decreases the slowest as the utility-loss budget increases and LRA-A has higher inference accuracies than other attacks except RF-A when the utility-loss budget is larger than 3. However, AttriGuard is still effective against LRA-A since LRA-A still has low  inference accuracies and approaches to the baseline attack as the utility-loss budget increases. %We believe it is an interesting future work to study noise detection both theoretically and empirically. 

\begin{figure}[!t]
%\vspace{-2mm}
\centering
%\subfloat[]{\includegraphics[width=0.45 \textwidth]{figs/Figure4/Figure4a.pdf}\label{up1}}
%\subfloat[]
{\includegraphics[scale=0.4]{figs/Figure4/Figure4-1.pdf}}
\caption{Impact of the target probability distribution. The attack is NN-A and the defender uses LR-D.} % \neil{Show inference accuracy as a function of utility-loss budget. One curve for $\mathbf{p}_u$, one curve for $\mathbf{p}_u$}}
%We observe that backtracking substantially improves VIAL's performance. }
%Second, we find that inference performances are stable across  different backtracking strengths once they are larger than 0.}
%\vspace{-4mm}
\label{tpd}
\end{figure}

\begin{figure}[t]
%\vspace{-2mm}
\centering
%\subfloat[]{\includegraphics[width=0.45 \textwidth]{figs/Figure4/Figure4a.pdf}\label{up1}}
%\subfloat[]
{\includegraphics[scale=0.4]{figs/Figure5/Figure5-1.pdf}}
\caption{Impact of the defender's classifier. The attack is NN-A.} %\neil{Show inference accuracy as a function of utility-loss budget. One curve for LR-D, one curve for NN-D}}
%We observe that backtracking substantially improves VIAL's performance. }
%Second, we find that inference performances are stable across  different backtracking strengths once they are larger than 0.}
%\vspace{-4mm}
\label{dclassifier}
\end{figure}

\myparatight{Impact of the target probability distribution} Figure~\ref{tpd} compares the performance of the two target probability distributions. We observe that the target probability distribution $\mathbf{p}_t$ outperforms $\mathbf{p}_u$, especially when the utility-loss budget is relatively large. 
Specifically, the attacker's inference accuracy is smaller when the defender uses $\mathbf{p}_t$.  This is because $\mathbf{p}_t$ considers the attribute information in the training dataset, while $\mathbf{p}_u$ assumes no knowledge about attributes. Specifically, according to our solution in Equation~\ref{ex1}, the defender adds the noise $\mathbf{r}_i$ with a probability that is the corresponding target probability normalized by the magnitude of $\mathbf{r}_i$. Suppose the defender's classifier predicts city $j$ for a user, where $j$ is likely to be the true attribute value of the user since the defender's classifier is relatively accurate.  The noise $\mathbf{r}_j$ is 0. Roughly speaking, if the defender adds 0 noise, then the attacker is likely to infer the true attribute value. For the users whose true attribute values are rare (i.e., small fraction of users have these attribute values), the defender is less likely to add 0 noise when using $\mathbf{p}_t$ than using $\mathbf{p}_u$. As a result, the attacker has a lower inference accuracy when $\mathbf{p}_t$ is used. 




\myparatight{Impact of the defender's classifier} Figure~\ref{dclassifier} shows the attacker's inference accuracy when the defender uses different classifiers, where the attack is NN-A. We observe that when the defender chooses the NN-D classifier, the attacker's inference accuracy is lower with the same utility-loss budget. One reason is that the noise found in Phase I is more likely to transfer between classifiers in the same category. Specifically, the noise optimized based on  NN-D is more likely to transfer to  NN-A than  LR-A. %Note that NN-D and NN-A have different neural network architectures.    

\begin{figure}[!t]
%\vspace{-2mm}
\centering
%\subfloat[]{\includegraphics[width=0.25 \textwidth]{figs/Figure6/Figure6c.pdf}\label{policy-pu}}
%\subfloat[]
{\includegraphics[scale=0.4]{figs/Figure7/Figure7-1.pdf}}
\caption{Impact of the overlap between the training datasets used by the attacker and the defender. }
%We observe that backtracking substantially improves VIAL's performance. }
%Second, we find that inference performances are stable across  different backtracking strengths once they are larger than 0.}
%\vspace{-4mm}
\label{training}
\end{figure}

\begin{figure}[!t]
%\vspace{-2mm}
\centering
%\subfloat[]{\includegraphics[width=0.25 \textwidth]{figs/Figure6/Figure6-1.pdf}\label{policy-pu}}
%\subfloat[]
{\includegraphics[scale=0.4]{figs/Figure6/Figure6-1.pdf}}
\caption{Impact of different noise-type-policies.} %\neil{Change y-axis to be Inference Accuracy.}}
%We observe that backtracking substantially improves VIAL's performance. }
%Second, we find that inference performances are stable across  different backtracking strengths once they are larger than 0.}
%\vspace{-4mm}
\label{policy}
\end{figure}




\myparatight{Impact of different training datasets} In practice, the attacker and the defender may use different training datasets to train their classifiers.  We randomly and evenly split the training dataset into two folds with $\alpha\%$ overlap, where $\alpha\%$ ranges from 0\% to 100\%. We consider the attack NN-A and use one fold to train the classifier, while we consider the defender's classifier is LR-D and use the other fold to train it. We set the utility-loss budget to be 4, which reduces most attacks to be close to the baseline attack. 
Figure~\ref{training} shows the attacker's inference accuracy as a function of the overlap $\alpha\%$. We find that the differences between the training datasets used by the attacker and the defender have impact on the effectiveness of AttriGuard, but the impact is small. Specifically, when the defender and the attacker use the same training dataset to learn their classifiers, the attacker's inference accuracy is around 0.10. The attacker's inference accuracy increases when the overlap between the training datasets decreases, but the attacker's inference accuracy is still less than 0.15 even if there are no overlaps. The reason is that both the attacker's classifier and the defender's classifier model the relationships between public data and attributes. Once both of their (different) training datasets are representative, the noise optimized based on the defender's classifier is very likely to transfer to the attacker's classifier. 


\myparatight{Impact of different noise-type-policies} Figure~\ref{policy} compares the three noise-type-policies. Modify\_Add outperforms Add\_New, which outperforms Modify\_Exist. This is because Modify\_Add is the most flexible policy, allowing AttriGuard to modify existing rating scores or add new rating scores.  A user often reviews a very small fraction of apps (e.g., 0.23\% of apps on average in our dataset), so Add\_New is more flexible than Modify\_Exist, making Add\_New outperform Modify\_Exist.


\begin{figure}[!t]
%\vspace{-2mm}
\centering
{\includegraphics[scale=0.4]{figs/Figure9/Figure9-1.pdf}}
\caption{Comparing AttriGuard with existing defense methods.}
%We observe that backtracking substantially improves VIAL's performance. }
%Second, we find that inference performances are stable across  different backtracking strengths once they are larger than 0.}
\vspace{-2mm}
\label{comparison}
\end{figure}

\myparatight{Comparing AttriGuard with existing defense methods} Figure~\ref{comparison} compares AttriGuard with existing defense methods developed by different research communities: BlurMe~\cite{weinsberg2012blurme}, ChiSquare~\cite{ChenObfuscationPETS14}, Quantization Probabilistic Mapping (QPM)~\cite{Salamatian:2015}, and Local Differential Privacy-Succinct Histogram (LDP-SH)~\cite{BassilySuccinctHistograms15}.  BlurMe and ChiSquare select the apps based on their correlations with the attribute values (i.e., cities in our case) that do not belong to the user and change the rating scores for the selected apps. QPM is an approximate solution to a game-theoretic formulation. We quantize public data to 200 clusters in QPM. 
LDP-SH is a local differential privacy method for categorical data. In our case, each entry of $\mathbf{x}$ can be viewed as categorical data taking values 0, 0.2, 0.4, 0.6, 0.8, or 1.0. We apply LDP-SH to each entry of $\mathbf{x}$.  We didn't use other LDP methods~\cite{Erlingsson:2014,Wang17LDP} because they do not preserve the semantics of rating scores. For instance, to obfuscate a user's rating score to an app, RAPPOR~\cite{Erlingsson:2014} might generate several rating scores for the app for the user, which is unrealistic. All the compared methods except LDP-SH use the same training dataset, while LDP-SH does not need training dataset. We note that BlurMe and ChiSquare require the defender to know users' true private attribute values.  

%Specifically, LDP-SH represents each entry $x_i$ as a 6-dimension vector $\mathbf{y}$, where an entry ${y}_j=$1 if and only if  $x_i=j$, where $j=0,1,2,3,4,5$. LDP-SH transforms the vector $\mathbf{y}$ using random projection and then randomly
%Due to limited space, we omit the details of these existing method, 


Each compared method has a parameter to control privacy-utility tradeoffs. 
For a method and a given parameter value, the method adds noise to users' public data, and we can obtain a pair (utility loss, inference accuracy), where the utility loss and inference accuracy are averaged over all test users. Therefore, for each method, 
via setting a list of different parameter values, we obtain a list of pairs (utility loss, inference accuracy). Then, we plot these pairs as a utility loss vs. inference accuracy curve. Figure~\ref{comparison} shows the curve for each method. 

Our AttriGuard outperforms all compared defense methods. Specifically, to achieve the same inference accuracy, AttriGuard adds substantially smaller noise to public data. AttriGuard outperforms BlurMe and ChiSquare because they add noise to entries of $\mathbf{x}$ that are selected based on heuristics, while AttriGuard adds minimum noise via solving optimization problems. %AttriGuard outperforms QPM because quantization changes public data substantially, which is equivalent to adding large noise. 
We explored a large range of the parameter to control privacy-utility tradeoffs for QPM, but QPM cannot reach to the low utility-loss region, i.e., we only observe a short curve for QPM in Figure~\ref{comparison}. This is because quantization changes public data substantially, which is equivalent to adding large noise. AttriGuard outperforms LDP-SH because LDP-SH aims to achieve a privacy goal that is different from defending against inference attacks.


 

\begin{figure}[!t]
%\vspace{-2mm}
\centering
{\includegraphics[scale=0.4]{figs/Figure11/Figure11-Precision.pdf}\label{recsys}}
\caption{Relative recommendation precision loss vs. top-$N$ recommendations.}
%We observe that backtracking substantially improves VIAL's performance. }
%Second, we find that inference performances are stable across  different backtracking strengths once they are larger than 0.}
\vspace{-2mm}
\label{recsys}
\end{figure}

\myparatight{Utility loss for recommender systems} We evaluate the utility loss of the public data when they are used for recommender systems. 
%The utility loss eventually should be evaluated by the quality loss of the service provided based on the noisy public data. 
%We empirically demonstrate that $L_0$ norm indeed well approximates service quality loss for reputation systems and recommender systems. 
For each user in the training and testing datasets, we randomly sample 5 of its rated apps to test a recommender system. We use a standard matrix factorization based recommender system to recommend top-$N$ items for each user. We implemented the recommender system using the code from http://surpriselib.com/. We measure the performance of the recommender system using a standard metric, i.e., \emph{recommendation precision}. For each user, the recommendation precision is the fraction of its recommended top-$N$ items that are among the sampled 5 rated apps. The recommendation precision for the entire recommender system is the recommendation precision averaged over all users.

%Before adding noise to the public data of the testing users, 
%we compute the average rating score for each item, which is the item's \emph{reputation score}. Moreover, for each user, we sample 5 of its rated apps uniformly at random. Then, we use a standard matrix factorization based recommender system to recommend top-$N$ items for each user. We implemented the recommender system using the code from http://surpriselib.com/. We measure the performance of the recommender system using a standard metric, i.e., \emph{recommendation precision}. For each user, the recommendation precision is the fraction of its recommended top-$N$ items that are among the sampled 5 rated apps. The recommendation precision for the entire recommender system is the recommendation precision averaged over all users.  

For each compared defense method, we use the defense method to add noise to the testing users, where the noise level is selected such that an attacker's inference accuracy is close to 0.1 (using the results in Figure~\ref{comparison}). 
Then, for each compared defense method, we compute the \emph{relative recommendation precision loss} defined as $\frac{|Pre_1 - Pre_2|}{Pre_1}$, where $Pre_1$ and $Pre_2$ are the recommendation precisions before and after adding noise, respectively.
 Figure~\ref{recsys} shows the {relative recommendation precision loss} as a function of $N$ for the compared methods. We observe AttriGuard outperforms the compared methods. Moreover, our results indicate that $L_0$ norm of the noise is a reasonable utility-loss metric for recommender systems, as a method with larger $L_0$-norm noise also has larger relative recommendation precision loss. One exception is the comparison between BlueMe and ChiSquare: ChiSquare adds noise with larger $L_0$ norm but has lower relative recommendation precision loss. This means that ChiSquare adds noise that is more similar to a user's public data and thus has less impact on a user's profile of preferences. 
 
 
%We add noise to the testing users using our AttriGuard with the utility-loss budget set to be 4. After adding noise, we re-compute the reputation score for each item and the recommendation precision for the recommender system. We find that the reputation score changes by only 0.03\% averaged over all items. %which means that our privacy protection mechanism has negligible impact on the utility of the public data when they are used for reputation systems. 
%Figure~\ref{recsys} shows the \emph{relative recommendation precision loss} as a function of $N$. The relative recommendation precision loss is defined as $\frac{|Pre_1 - Pre_2|}{Pre_1}$, where $Pre_1$ and $Pre_2$ are the recommendation precisions before and after adding noise, respectively. We observe that the relative recommendation precision loss is small, i.e., less than 3\%. 
%Our results show that AttriGuard incurs small utility loss in the context of reputation and recommender systems. 
% Recommender system has a larger utility loss than reputation system. This is because recommender system relies on the complex correlations between rating scores, while reputation system simply relies on items' average rating scores. 

 %We note that the results correspond to a strong privacy protection, i.e., the privacy-budget is set to be 0.2. If users can tolerate a lager




